Stochastic Methods in Variational Inequalities: Ergodicity, Bias and Refinements

For min-max optimization and variational inequalities problems (VIP) encountered in diverse machine learning tasks, Stochastic Extragradient (SEG) and Stochastic Gradient Descent Ascent (SGDA) have emerged as preeminent algorithms. Constant step-size variants of SEG/SGDA have gained popularity, with appealing benefits such as easy tuning and rapid forgiveness of initial conditions, but their convergence behaviors are more complicated even in rudimentary bilinear models. Our work endeavors to elucidate and quantify the probabilistic structures intrinsic to these algorithms. By recasting the constant step-size SEG/SGDA as time-homogeneous Markov Chains, we establish a first-of-its-kind Law of Large Numbers and a Central Limit Theorem, demonstrating that the average iterate is asymptotically normal with a unique invariant distribution for an extensive range of monotone and non-monotone VIPs. Specializing to convex-concave min-max optimization, we characterize the relationship between the step-size and the induced bias with respect to the Von-Neumann's value. Finally, we establish that Richardson-Romberg extrapolation can improve proximity of the average iterate to the global solution for VIPs. Our probabilistic analysis, underpinned by experiments corroborating our theoretical discoveries, harnesses techniques from optimization, Markov chains, and operator theory.

==> Body/Experiments.tex <==
% !TEX root = ../Arxiv-Main.tex


In this section, we conduct the following series of experiments to empirically observe and validate our results. We focus on a strongly convex-concave game with two players. See the appendix for the details of experiments, for which we have adapted the code of the repository of~\cite{HIMM20}.


\begin{figure}[t]
\centering
\begin{subfigure}[b]{.38\linewidth}
\includegraphics[width=\textwidth]{./figures/figure_GD_bias.png}
\caption{SGDA.}
\label{fig:GD_bias}
\end{subfigure}%
%
\begin{subfigure}[b]{.38\linewidth}
\includegraphics[width=\textwidth]{./figures/figure_EG_bias.png}%
\caption{SEG.}
\label{fig:EG_bias}
\end{subfigure}

\caption{Convergence and bias under different step-sizes for SGDA and SEG.}
\label{fig:bias}
\end{figure}

We started by plotting in \cref{fig:GD_bias,fig:EG_bias} the error $\norm{\state -\sol}^2$ for both  \eqref{eq:SGDA}, \eqref{eq:SEG} for step-sizes $\gamma \in \{0.1 , 0.05 , 0.01 , 0.001\}$, corresponding to the four curves from top to bottom; the value of $\stepalt$ was set to $0.5$.  We observe  a decay of the bias as a function of the step-size (the decay is in fact almost linear for both algorithms).  

\begin{figure}[h]
\centering
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=0.8\textwidth]{./figures/fewiter-0.005-100-2000.png}%
\caption{SGDA}
\label{fig:SGDA-diff}
\end{subfigure}%
%
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=0.8\textwidth]{./figures/fewiter-EG-0.005-100-2000.png}%
\caption{SEG}
\label{fig:SEG-diff}
\end{subfigure}
\caption{Results for $100$  (light purple), $200$ (light green), $1000$ (light blue) iterations (or from right to left).}
\label{fig:normal-different-iterations}
\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=0.8\textwidth]{./figures/GD-two.png}%
\caption{SGDA}
\label{fig:SGDA-steps}
\end{subfigure}%
%
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=0.8\textwidth]{./figures/EG-two.png}%
\caption{SEG}
\label{fig:SEG-steps}
\end{subfigure}
\caption{Histograms for two different step-sizes. Green: $\gamma = 0.1$. Purple: $\gamma = 0.001$.}
\label{fig:normal-steps}
\end{figure}
The second set of experiments examines the central limit theorem (CLT). We use as test function the value of the game, which is zero, and we observe the behavior of its averaged evaluations after  $100,200$ and $1000$ iterations. To do so we run both algorithms with step-size $\step = 0.005$ for the aforementioned number of iterations and keep the sum of the evaluations, normalized with $\sqrt{\text{iterations}}$. We repeat this experiment 2000 times and report the histograms in \cref{fig:normal-different-iterations}. We observe how the distributions are concentrated closer to the actual value of the game as the number of iterations is increased. In \cref{fig:normal-steps} we run both algorithms in the previous setting for 1000 iterations and two different step-sizes $0.1$ and $0.001$. We observe how the histogram is concentrated closer to the actual value of the game for smaller step-size.





==> Body/Introduction.tex <==
%----------------------------------------------------------------------
%%% INTRODUCTION
%----------------------------------------------------------------------
% !TEX root = ../Arxiv-Main.tex

Variational inequalities problem (VIP) is a versatile framework that incorporates a broad range of problems including loss minimization, min-max optimization, bilinear games and various fixed point problems. Many problems in machine learning, such as training Generative Adversarial Networks (GANs) \cite{goodfellow_2014_gan}, Actor-Critic methods \cite{pfau2016connecting}, multi-agent reinforcement learning \cite{zhang2021multi} and robust learning \cite{wen2014robust}, can be cast as VIPs. 

In many applications of VIP, one is  given only a stochastic oracle, typically constructed from finite data, that provides noisy access to the underlying operator. Various stochastic algorithms for VIP have been proposed and analyzed, with two prime examples being Stochastic Extragradient (SEG) \cite{juditsky2011solving} and Stochastic Gradient Descent Ascent (SGDA) methods~\cite{nemirovski2009robust}. It has been well recognized that convergence properties of stochastic VIP methods are more delicate than their deterministic and loss minimization counterparts. Nevertheless, much progress has been made in recent years, on both SEG \cite{mishchenko2020revisiting,kannan2019optimal,mertikopoulos2019learning,HIMM20,beznosikov2020distributed,gorbunov2022stochastic} and SGDA \cite{nemirovski2009robust,loizou2021stochastic,yang2020global,lin2020finite, beznosikov2023stochastic}. The  closely related stochastic gradient descent (SGD) method~\cite{gorbunov2020unified}, which can be viewed as a special case of SGDA, has an even larger and still growing literature. Classical results on these stochastic methods typically assume that a diminishing step-size is used, which allows for last-iterate convergence to the global solution~\cite{Polyak92-Avg,Douc2018,kushner2003-yin-sa-book,Benveniste12-sa-book}.

In this paper, we focus on the constant step-size variants of SEG and SGDA. Constant step-sizes are popular in practice, with several major benefits: the resulting algorithm is easy to tune with only a single parameter; it is insensitive to the initial condition, which is forgotten quickly; the algorithm makes substantial progress even in the first few iterations. Empirically, the use of constant step-size often leads to good performance in practical machine learning tasks and beyond.

The analysis of constant step-size SEG and SGDA, however, is more complicated, with various non-convergent behaviors even in rudimentary bilinear models \cite{gidel2018variational,mertikopoulos2019optimistic,chavdarova2019reducing,HIMM20,daskalakis2018training}. In particular, similar to SGD \cite{Dieuleveut20-bach-SGD}, these algorithms in general do not converge to the exact solution of the VIP. Rather, due to stochastic noise, the iterates fluctuate within a neighborhood of the solution.  Existing theoretical results are typically in the form of an \emph{upper bound} on the mean squared error or dual gap of the iterations. Such upper bounds often compound the deterministic and stochastic aspects of the convergence behavior.


In this work, we seek to elucidate and quantify the behaviors of SEG and SGDA with constant step-sizes. Rather than treating the stochastic fluctuation as a nuisance, we fully embrace the probabilistic nature of SEG and SGDA. By viewing them as time-homogeneous Markov chains, we study their fine-grained distributional properties, disentangling the deterministic and stochastic components. In particular, we show that while the iterate does not converge, its distribution does. Moreover, this perspective allows us to use the information provided by their fluctuation for uncertainty quantification.

\para{Our contributions} 
We consider a class of VIPs with weak quasi strongly monotonicity, which encompasses a broad range of structured non-monotone and non-convex problems. Under appropriate regularity assumptions, we establish the following results.
\begin{itemize}[topsep=0pt,itemsep=0ex,leftmargin=15pt]
    \item We prove that the iterates of SEG and SGDA form a Harris and positive recurrent Markov chain, which admits a unique stationary distribution. Our results quantify the relationship between the step-size and the regularity parameters of the VIP for ensuring recurrence.
    \item We show that the distribution of the iterates converges geometrically to the above stationary distribution. More generally, we establish geometric convergence of the expectation of any Lipschitz test function of the iterates.
    \item We derive an ergodic Law of Large Number and a Central Limit Theorem for the iterates, thereby establishing the asymptotic normality of the ergodic average of the iterates.
    \item We show that induced bias---the distance between the mean of the stationary distribution and the global solution of the VIP---is bounded by a linear function of the step-size and the weak monotonicity parameter. Specializing to convex-concave min-max optimization, we quantify the relationship between the step-size and the bias with respect to the Von-Neumann’s value.
    \item For SGDA applied to quasi strongly monotone VIPs, we derive a first-order expansion of the induced bias in terms of the step-size. This characterization shows that an order-wise reduction the bias of SGDA can be achieved by the Richardson-Romberg refinement scheme.
\end{itemize}

\subsection{Related work}

Below we review prior work on VIP with a focus on stochastic methods with constant step-sizes.

\para{Variational Inequalities} VIP and its various special cases has been studied extensively, especially in the deterministic setting where one has exact access to the operator. Many algorithms have been developed, with both asymptotic convergence and finite-time guarantees. It is beyond the scope of this paper to survey these results, but we mention that for VIPs with Lipschitz
continuous and monotone operator, the works \cite{nemirovski2004prox} study a variant of Extra Gradient algorithm \cite{Kor76} and establishes optimal convergence rates for ergodic average, and the work \cite{gidel2018variational,mokhtari2020unified} studies proximal point algorithm with geometric
convergence results.

Most related to us are works for the stochastic setting, for which SEG \cite{juditsky2011solving}
and SGDA \cite{nemirovski2009robust} are two of the most prominent algorithms. Non-convergent phenomena are observed even in  unconstrained
bilinear games \cite{gidel2018variational,mertikopoulos2019optimistic,chavdarova2019reducing,daskalakis2018training,HIMM20}. 
Complementarily, a growing line of work has been dedicated to better
understanding of SEG and SGDA and bridging the gap
between the deterministic and the stochastic cases. The work \cite{juditsky2011solving}
provided the first analysis of SEG for monotone VIPs. Subsequent
work has extended these results to other settings \cite{mishchenko2020revisiting,kannan2019optimal,mertikopoulos2019learning,HIMM20,beznosikov2020distributed,gorbunov2022stochastic}.
A parallel line of work studies SGDA and its variants under different scenarios
\cite{nemirovski2009robust,loizou2021stochastic,yang2020global,lin2020finite}.
Recently \cite{beznosikov2023stochastic} proposed a unified convergence
analysis that covers various SGDA methods for regularized VIPs, where
the operator is either quasi-strongly monotone or $\ell$-star-cocoercive.
For a quantitative summary of existing results, we refer the readers to \cite{gorbunov2022stochastic} for SEG and \cite{beznosikov2023stochastic} for SGDA.

In this paper we consider \emph{weakly quasi-strongly monotone} VIPs, which is a class
of structured non-monotone operators under which one can bypass the
the intractability issue that arises in general non-monotone regime
\cite{diakonikolas2021efficient,daskalakis2021complexity,kakutani2hard}. Similar
conditions have been considered in prior work to establish the convergence
guarantee of various algorithms \cite{HIMM20,gorbunov2022stochastic,yang2020global,song2020optimistic,loizou2021stochastic}.



\para{Constant step-size SGD and Stochastic Approximation}

The literature on SGD and stochastic approximation (SA) is vast. Within this literature, our work is most related to, and in fact motivated by, a recent line of work that studies constant step-size SGD and SA through the lens of stochastic processes. The work \cite{Dieuleveut20-bach-SGD} studies SGD for smooth and strongly
convex functions. Extensions to non-convex functions are considered in 
\cite{Yu21-stan-SGD}, which establishes a central limit theorem that is similar in spirit to our results. More recently, \cite{bianchi2022convergence} studies SGD for non-smooth non-convex functions. 
The work \cite{durmus2021riemannian} considers constant step-size SA on Riemannian
manifolds and studies the limiting behavior as the step-size approaches zero. The work \cite{huo21-td} considers linear SA with Markovian noise; see the references therein for other recent results on SA. We mention that both \cite{Dieuleveut20-bach-SGD} and  \cite{huo21-td} examine the Richardson-Romberg bias refinement scheme, which we also consider in this paper.


